Extension of derivations, and Connes-amenability of the enveloping dual Banach algebra

If $D:A \to X$ is a derivation from a Banach algebra to a contractive, Banach $A$-bimodule, then one can equip $X^{**}$ with an $A^{**}$-bimodule structure, such that the second transpose $D^{**}: A^{**} \to X^{**}$ is again a derivation. We prove an analogous extension result, where $A^{**}$ is replaced by $\F(A)$, the \emph{enveloping dual Banach algebra} of $A$, and $X^{**}$ by an appropriate kind of universal, enveloping, normal dual bimodule of $X$. Using this, we obtain some new characterizations of Connes-amenability of $\F(A)$. In particular we show that $\F(A)$ is Connes-amenable if and only if $A$ admits a so-called WAP-virtual diagonal. We show that when $A=L^1(G)$, existence of a WAP-virtual diagonal is equivalent to the existence of a virtual diagonal in the usual sense. Our approach does not involve invariant means for $G$.

==> WAPmac8.tex <==
% Call this AFTER the macros that are specific to the personal or the MathScand versions


%-------- diagrams -- needs Paul Taylor's macros
\NeedsTeXFormat{LaTeX2e}
% load up Paul Taylor's diagram.sty macros

\RequirePackage[PS,nohug]{diagrams}
% this should now avoid annoying label rotation


%% Arrow definitions
\newarrowmiddle{o}{\circ}{\circ}{\circ}{\circ}
%\newarrowmiddle{.}{\bullet}{\bullet}{\bullet}{\bullet}

\newarrow{Eq} ===== % identity map/morphism
\newarrow{Dash} {}{dash}{}{dash}>
\newarrow{Dots} ....>

\newcommand{\ackndiag}{Uses Paul Taylor's \texttt{diagrams.sty} macros}

%------------------

% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{YCnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}
\numberwithin{equation}{section}


\newcommand{\defeq}{:=}
\newcommand{\st}{\mathbin{\colon}}

%-------- WORKAROUND FOR JOURNAL CONVENTION

% in preprint version bbrd will be an alias for mathbb
% in MathScand version it will be an alias for mathsf
% (following house style)

% \newcommand{\C}{\bbrd{C}}
\newcommand{\Cplx}{{\bbrd C}}
\newcommand{\T}{\bbrd{T}}
\newcommand{\Nat}{{\bbrd N}}
\newcommand{\Z}{{\bbrd Z}}

%------------------


% TRIANGULAR BANACH ALGEBRA
% try alternative notation (Oct 2012)
\newcommand{\TR}[2]{{#1}\oplus_{\ltimes}{#2}}
\newcommand{\TAX}{\TR{A}{X}}

\newcommand{\pcat}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\BAlg}{\pcat{BAlg}}
\newcommand{\Der}{\operatorname{\mathsf{Der}}}


\newcommand{\iso}{\cong}
\newcommand{\lin}{\operatorname{lin}}

\newcommand{\wstar}{\ensuremath{{\rm w}^*}}
\newcommand{\sid}{\operatorname{id}\nolimits}

\newcommand{\blank}{\underline{\quad}}


\newcommand{\Cst}{\ensuremath{\operatorname{C}\nolimits^*}}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}
\newcommand{\norm}[1]{\Vert#1\Vert}

\newcommand{\Lin}{{\mathcal L}}

\newcommand{\tp}{\mathbin{\otimes}}
\newcommand{\ptp}{\mathbin{\widehat{\otimes}}}

\newcommand{\wtild}[1]{\widetilde{#1}}
\newcommand{\pair}[2]{\langle{#1},\,{#2}\rangle}

%\newcommand{\Arp}{\mathbin{\scriptstyle\square}}
\newcommand{\Arp}{\mathbin{\scriptscriptstyle\square}} % Ross prefers them smaller

\newcommand{\wslim}{\hbox{{\rm w}${}^*$-}\lim}
\newcommand{\id}[1][]{{1}_{#1}}

\newcommand{\tmat}[2]{\left[\begin{matrix} #1 & #2 \\ 0 & #1 \end{matrix}\right]}


% lazy YC abbreviations -- text

\newcommand{\ibid}{{\it ibid.}\/}
%\newcommand{\ndb}{ndb}  % normal dual Banach
\newcommand{\hm}{homomorphism}
\newcommand{\wswscts}{\wstar-\wstar\ continuous}
\newcommand{\KS}{Krein-\v{S}mulian}

% lazy YC abbreviations -- math
\newcommand{\til}[1]{\widetilde{#1}}
\renewcommand{\AA}{A\ptp A}

% abbreviations for greek
\newcommand{\gm}{\gamma}
\newcommand{\Gm}{\Gamma}
\newcommand{\kp}{\kappa}

\newcommand{\veps}{\varepsilon}


% various physical markup
\newcommand{\sg}{{\bf g}}
\newcommand{\sh}{{\bf h}}
% \newcommand{\sJ}{{\mathsf J}}



%\newcommand{\cA}{{\mathcal A}}
%\newcommand{\cB}{{\mathcal B}}
%\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cT}{{\mathcal T}}
%\newcommand{\cU}{{\mathcal U}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%% NOTATION FOR DBAs

%%% Elements of normal dual modules, in particular the free ones

% idea was to use fraktur for elements of WAP-star-star
% previously this was tilde
% now leaning towards bold sans serif

% \newcommand{\ndm}[1]{\widetilde{#1}}   % for elements of the free DBA
%\newcommand{\ndm}[1]{{\mathfrak#1}}
\newcommand{\ndm}[1]{{\textbf{\textsf{#1}}}}

\newcommand{\tila}{\ndm{a}}
\newcommand{\tilb}{\ndm{b}} % tweaks by YC to avoid macro clash
\newcommand{\tilc}{\ndm{c}}
\newcommand{\tile}{\ndm{e}}
\newcommand{\tilf}{\ndm{f}}
\newcommand{\tilg}{\ndm{g}}
%\newcommand{\tilh}{\ndm{h}}
\newcommand{\tilm}{\ndm{m}}
\newcommand{\tiln}{\ndm{n}}
\newcommand{\tils}{\ndm{s}}
\newcommand{\tilw}{\ndm{w}}
\newcommand{\tilx}{\ndm{x}}
\newcommand{\tily}{\ndm{y}}
\newcommand{\tilth}{\widetilde{\theta}}
%% \newcommand{\tilthet}{\widetilde{\theta}}

%% notation for normal dual modules/dual Banach algebras
\newcommand{\nor}[1]{{\mathsf #1}}
\newcommand{\fB}{\nor{B}}
\newcommand{\fM}{\nor{M}}
\newcommand{\fN}{\nor{N}}
\newcommand{\fX}{\nor{X}}

% WAP extensions of maps
\newcommand{\gwap}{g_{\WAP}}
\newcommand{\hwap}{h_{\WAP}}
\newcommand{\Dtild}{\widetilde{D}}
\newcommand{\DWAP}{\Delta_{\WAP}}
\newcommand{\DW}{\Delta_{\WAP}}

% images in WAPstarstar of elements in original module or algebra
% macros renamed by YC
%\newcommand{\bv}{\breve}
%\newcommand{\bre}[1]{({#1})^{\breve{}}}

% changed by YC as the breves don't look so good IMHO
\newcommand{\bv}[1]{\overline{#1}} 
\newcommand{\bre}[1]{\overline{#1}}



\newcommand{\ba}{\bv{a}}
\newcommand{\bb}{\bv{b}}
\newcommand{\bc}{\bv{c}}
\newcommand{\bw}{\bv{w}}
\newcommand{\bx}{\bv{x}}
\newcommand{\by}{\bv{y}}
\newcommand{\bm}{\bv{m}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Meta symbols
\newcommand{\SC}{\operatorname{SC}}
\newcommand{\CB}{\operatorname{CB}}
\newcommand{\UC}{\operatorname{UC}}
\newcommand{\UCB}{\operatorname{UCB}}
\newcommand{\LUC}{\operatorname{LUC}}

\newcommand{\WAP}{\ensuremath{\operatorname{WAP}}}  % for use in inline text, etc
\newcommand{\LWAP}{\operatorname{LWAP}}
\newcommand{\RWAP}{\operatorname{RWAP}}


%% Volker's sigma-WC
\newcommand{\sigWC}{\sigma{\rm WC}}


%% Free DBAs, free normal dual modules
\newcommand{\basewap}[1]{{\,}_{#1}{\rm WAP}_{#1}}
\newcommand{\AWAPA}{\basewap{A}}
\newcommand{\fBWAPfB}{\basewap{\fB}}



%\newcommand{\F}{{\mathcal F}}
%\newcommand{\F}{{\mathfrak F}}
\newcommand{\F}{\nor{F}} % have settled on sans serif for free functor, fits above notation for normal modules
\newcommand{\FA}{\F(A)}
\newcommand{\FT}{\F(T)}
\newcommand{\FAN}{\F_A(N)}
\newcommand{\FAX}{\F_A(X)}
\newcommand{\FAY}{\F_A(Y)}
\newcommand{\FAZ}{\F_A(Z)}
\newcommand{\FAWAPFA}{\basewap{{\F(A)}}} % irritating but needed in one place
\newcommand{\LGWAPLG}{\basewap{L^1(G)}}

\newcommand{\SWAP}{{\rm SWAP}}
\newcommand{\ewap}{e_{\rm WAP}} % alternative notation for identity element in F(A)


\newcommand{\DERFA}{{\F}\pcat{DER}_A}
\newcommand{\DERA}{\pcat{DER}_A}

% Function spaces on G
\newcommand{\CBG}{\operatorname{CB}(G)}
\newcommand{\WAPG}{\WAP(G)}
\newcommand{\LUCG}{\LUC(G)}
\newcommand{\LG}{L^1(G)}
\newcommand{\LIG}{L^\infty(G)}
\newcommand{\LGop}{L^1(G^{\rm op})}


% misc grammar
\newcommand{\ess}{{\rm ess}} % just to save me having to write it all the time

% Function spaces on G\times G
\newcommand{\GG}{G \times G}
\newcommand{\Gop}{G^{\rm op}}
\newcommand{\GGop}{G\times \Gop}

% descriptive names
\newcommand{\LUCGGOP}{\LUC(\GGop)}
\newcommand{\CBGG}{\CB(\GG)}
\newcommand{\GWAPG}{{\,}_G{\rm \WAP}_G(\GG)}
\newcommand{\SWAPS}{{\,}_S{\rm \WAP}_S(S\times S)}
\newcommand{\LWAPL}{{\,}_{\LG}{\rm WAP}_{\LG}(\LIGG)}

\newcommand{\LGG}{L^1(\GG)}
\newcommand{\LIGG}{L^\infty(\GG)}
%\newcommand{\DG}{{\Delta_G}}
%\newcommand{\DGO}{\Delta_{G^o}}

\newcommand{\Nmin}{{\Nat}_{\min}}


% ad hoc symbols
\newcommand{\cV}{{\mathcal V}}
%\newcommand{\LUCR}{\operatorname{\bf LUCR}}
\newcommand{\LUCR}{{\mathcal U}}
\newcommand{\cU}{{\mathcal U}} % stands for LUC(G\times G^{op})
%\newcommand{\LWAPR}{\operatorname{\bf LWAPR}}
%\newcommand{\LWAPR}{{\mathcal W}}

\newcommand{\cW}{{\mathcal W}} % stands for L^1(G)-WAP(L^\infty(G\times G))-L^1(G)


==> WAPmac_pers.tex <==
% called BEFORE the common macros
\usepackage[usenames]{color}
%\newcommand{\YCnote}[1]{\textcolor{Blue}{[\textsf{#1}]}}


\usepackage{amsmath,amsfonts,amssymb,amsthm}

\usepackage{sectsty}
%\allsectionsfont{\sffamily}
\allsectionsfont{\sc}

\setlength{\textheight}{22cm} \setlength{\textwidth}{15cm}
\setlength{\voffset}{-2.5cm} \setlength{\hoffset}{-.85cm}
\setlength{\topmargin}{1cm}
\parskip=0.2em


% ------------------------------

% YC's approach to theorem environments

\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse


% Styles for theorems, definitions, remarks

\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem*{notn}{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}
\newtheorem{remark}[pulse]{Remarks}
\newtheorem{ex}[pulse]{Example}
\newtheorem{question}[pulse]{Question}

%%%%%%%


% Specific deviations from journal style

\newcommand{\dt}[1]{\textcolor{Maroon}{\it#1}\/}

\newcommand{\bbrd}{\mathbb} 



